Scallop: A Language for Neurosymbolic Programming

We present Scallop, a language which combines the benefits of deep learning and logical reasoning. Scallop enables users to write a wide range of neurosymbolic applications and train them in a data- and compute-efficient manner. It achieves these goals through three key features: 1) a flexible symbolic representation that is based on the relational data model; 2) a declarative logic programming language that is based on Datalog and supports recursion, aggregation, and negation; and 3) a framework for automatic and efficient differentiable reasoning that is based on the theory of provenance semirings. We evaluate Scallop on a suite of eight neurosymbolic applications from the literature. Our evaluation demonstrates that Scallop is capable of expressing algorithmic reasoning in diverse and challenging AI tasks, provides a succinct interface for machine learning programmers to integrate logical domain knowledge, and yields solutions that are comparable or superior to state-of-the-art models in terms of accuracy. Furthermore, Scallop's solutions outperform these models in aspects such as runtime and data efficiency, interpretability, and generalizability.

==> figures/benchmark-summary.tex <==
\begin{table}
    \footnotesize
    \centering
    \begin{tabular}{c|c||c|c|c|c|c|c|c}
        \toprule \hline
        Task & Subtask & Domain & Focus & Rec. & Neg. & Agg. & LoC (.py) & LoC (.scl) \\ \hline
        \multirow{4}{*}{MNIST-R} & $\text{sum}_{2,3,4}$ & CV & Arithmetic & & & & 223 & 3 \\
                                 & $\text{sort}_{2,3}$ & CV & Comparison & & & & 228 & 3 \\
                                 & $\text{not}_{3,4}$ & CV & Negation & & \ding{52} & & 195 & 2 \\
                                 & $\text{count}_{10}$ & CV & Aggregation & & \ding{52} & \ding{52} & 231 & 2 \\
        \hline
        HWF & -- & CV & Parsing \& Evaluation & \ding{52} & & & 281 & 41 \\
        \hline
        \multirow{2}{*}{Pathfinder} & PATH & CV & Long Range & \ding{52} & & & 265 & 4 \\
                                    & PATH-X & CV & Long Range & \ding{52} & & & 265 & 4 \\
        \hline
        \multirow{3}{*}{CLUTRR} & RE & NL & Relation Extraction & \ding{52} & & & 460 & 152 \\
                                & RL & NL & Rule Learning & \ding{52} & & & 299 & 8 \\
                                & RE-RL & NL & Rel. Ext. + Rule Learning & \ding{52} & & & 504 & 8 \\
        \hline
        \multirow{2}{*}{CLEVR} & VO-Count & CV & Scene Graph + Count & & \ding{52} & \ding{52} & 162 & 53 \\
                               & VO & CV & Scene Graph + DSL Interpreter & \ding{52} & \ding{52} & \ding{52} & 851 & 53 \\
                            %    & QO & NL & Semantic Parsing & \ding{52} & \ding{52} & \ding{52} & & 50 \\ \hline
        \hline
        VQAR & -- & CV & Scene Graph + Knowledge Graph & \ding{52} & & & \\
        \hline \bottomrule
    \end{tabular}
    \caption{
        Characteristics of our benchmark tasks and statistics of their solutions expressed using \ours. \mayur{In first column, also cite the paper where this task was originally proposed.}
    }
    \label{tab:benchmark-summary}
\end{table}


==> figures/diff-top-k-proofs-def.tex <==
% \begin{figure}
%   \footnotesize
%   \[
%     \arraycolsep=3pt
%     \begin{array}{rrcl}
%       \text{(Variable)} & i & \in & 1 \dots n \\
%       \text{(Literal)} & \nu & ::= & \text{pos}(i) \sep \text{neg}(i) \\
%       \text{(Proof)} & \eta & ::= & \{ \nu_1, \nu_2, \dots \} \\
%       \text{(Formula)} & \Phi \ni \varphi & ::= & \{ \eta_1, \eta_2, \dots \}
%     \end{array}
%     \quad
%     \begin{array}{rcl}
%       \varphi_1 \vee_k \varphi_2 & = & \text{top}_k(\varphi_1 \cup \varphi_2) \\
%       \varphi_1 \wedge_k \varphi_2 & = & \text{top}_k(\{ \eta \sep \eta = \eta_1 \cup \eta_2, \eta ~\text{no conflict}, (\eta_1, \eta_2) \in \varphi_1 \times \varphi_2 \}) \\
%       \neg_k~ \varphi & = & \text{top}_k(\text{cnf2dnf}(\{ \{\neg \nu \sep \nu \in \eta \} \sep \eta \in \varphi \})) \\
%       \Gamma(i) & = & (r_i, \vec{\mathbf{e}}_i)
%     \end{array}
%   \]
%   \caption{Definitions of \inlinecodesmall{diff-top-k-proofs} (\inlinecodesmall{dtkp})}
%   \label{fig:top-k-proofs-def}
%   \Description{}
% \end{figure}


==> figures/hwf-data-efficiency.tex <==
\begin{figure}
  \centering
  \footnotesize
  \begin{tabular}{c||c|c|c|c}
    \multirow{2}{*}{\%Train} & \ours & \multicolumn{3}{c}{NGS} \\ \cline{2-5}
    & \texttt{dtkp-5} & RL & MAPO & $m$-BS \\ \hline
    100\% & 97.85 & 3.4 & 71.7 & 98.5 \\ \hline
    50\% & 95.7 & 3.6 & 9.5 & 95.7 \\ \hline
    25\% & 92.95 & 3.5 & 5.1 & 93.3 \\
  \end{tabular}
  \caption{
    Testing accuracy of various methods on HWF when training on only a portion of the data.
    Numbers are in percentage (\%)}
  \label{fig:hwf-data-efficiency}
  \Description{}
\end{figure}


==> figures/hwf-runtime.tex <==
\centering
\footnotesize
\begin{tabular}{c|c}
    \toprule \hline
    Provenance & Runtime (s) \\ \hline
    \texttt{maxminprob} & 101 \\
    \texttt{top3proofs} & 127 \\
    \texttt{top5proofs} & 152 \\ \hline
    \bottomrule
\end{tabular}
% \captionof{figure}{Avg. runtime per epoch}
\label{table:hwf-runtime}


==> figures/interp-gene-data-effi.tex <==
% \begin{figure}
%   \begin{minipage}[t]{0.48\textwidth}
%     \centering
%     \footnotesize
%     \begin{tabular}{ccc}
%       \includegraphics[width=0.7in]{images/MUGEN/MUGEN-climb-ladder.jpg} &
%       \includegraphics[width=0.7in]{images/MUGEN/MUGEN-collect-coin.jpg} &
%       \includegraphics[width=0.7in]{images/MUGEN/MUGEN-kill-face.jpg} \\
%       \inlinescl{(climb,up)} &
%       \inlinescl{(collect,coin)} &
%       \inlinescl{(kill,face)}
%     \end{tabular}
%     \captionof{figure}{
%       The predicted most likely (action, mod) pair for example video segments from Mugen dataset.
%     }
%     \label{fig:mugen-interpretability}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[t]{0.48\textwidth}
%     \centering
%     \footnotesize
%     \begin{tabular}{c||c|c|c|c}
%       \multirow{2}{*}{\textbf{\%Train}} & \textbf{\ours} & \multicolumn{3}{c}{\textbf{NGS}} \\ \cline{2-5}
%       & \texttt{dtkp-5} & RL & MAPO & $m$-BS \\ \hline
%       100\% & 97.85 & 3.4 & 71.7 & 98.5 \\ \hline
%       50\% & 95.7 & 3.6 & 9.5 & 95.7 \\ \hline
%       25\% & 92.95 & 3.5 & 5.1 & 93.3 \\
%     \end{tabular}
%     \vspace{6.5px}
%     \captionof{table}{
%       Testing accuracy of various methods on HWF when trained with only a portion of the data.
%       Numbers are in percentage (\%).}
%     \label{tab:hwf-data-efficiency}
%   \end{minipage}
% \end{figure}


==> figures/interpretability-mugen.tex <==
\begin{minipage}{\textwidth}
  \centering
  \footnotesize
  \begin{tabular}{ccc}
    \inlinescl{(19,climb,up)} &
    \inlinescl{(12,collect,coin)} &
    \inlinescl{(25,kill,face)} \\
    \includegraphics[width=0.12\textwidth]{images/MUGEN/MUGEN-climb-ladder.jpg} & \includegraphics[width=0.12\textwidth]{images/MUGEN/MUGEN-collect-coin.jpg} & \includegraphics[width=0.12\textwidth]{images/MUGEN/MUGEN-kill-face.jpg}
  \end{tabular}
  \captionof{figure}{The most likely predicted actions}
\end{minipage}


==> figures/pacman-illustration.tex <==
\begin{figure}
  \centering
  \begin{subfigure}[h]{0.3\linewidth}
      \centering
      \includegraphics[width=0.95\linewidth]{figures/pacman-1}
      \caption{Step 0}
      \label{fig:pacman-1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[h]{0.3\linewidth}
      \centering
      \includegraphics[width=0.95\linewidth]{figures/pacman-2}
      \caption{Step 4}
      \label{fig:pacman-2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[h]{0.3\linewidth}
      \centering
      \includegraphics[width=0.95\linewidth]{figures/pacman-3}
      \caption{Step 7}
      \label{fig:pacman-3}
  \end{subfigure}
%   \hfill
%   \begin{subfigure}[h]{0.24\textwidth}
%       \centering
%       \includegraphics[width=0.8\textwidth]{figures/pacman-overlay-30}
%       \caption{overlayed predictions}
%       \label{fig:pacman-overlay-30}
%   \end{subfigure}
  \caption{
      3 states of one gameplay session.
      States are overlaid to visualize progression.
    %   In Fig. \ref{fig:pacman-overlay-30}, we visualize what the neural network predicts over each cell after 30 training episodes: {\color{red} enemy}, {\color{blue} agent}, {\color{sclgreen} goal}.
  }
  \label{fig:avoiding-enemy-demo}
\end{figure}


==> figures/pacman-learning.tex <==
\begin{wrapfigure}{r}{0.40\textwidth}
  \begin{subfigure}[h]{0.48\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/pacman-overlay-5}
    \caption{5th episode}
    \label{fig:pacman-overlay-5}
  \end{subfigure}
  \hfill
  \begin{subfigure}[h]{0.48\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/pacman-overlay-15}
    \caption{15th episode}
    \label{fig:pacman-overlay-15}
  \end{subfigure}
  \caption{
    Overlaid predictions in 5th and 15th training episodes:
    {\color{red} enemy}, {\color{blue} agent}, {\color{sclgreen} goal}.
  }
  \label{fig:pacman-overlay-5-15}
\end{wrapfigure}


==> figures/pacman-pipeline.tex <==
% https://drive.google.com/file/d/1lft_lSM5nIaGlu5PPQt4u-swi81RL8m9/view?usp=sharing
\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{figures/scallop-program-pipeline.pdf}
  \caption{Dataflow diagram of a \ours~ program. \todo{There is something unsatisfying about this diagram: the pacman example has a feedback loop which is not reflected here. Not sure how to fix.}}
  \label{fig:scallop-program-pipeline}
  \vspace{-0.1in}
\end{figure}
% TODO: the image in the background of the pac-man problem may be copyrighted


==> figures/runtime-efficiency.tex <==
\begin{table}
  \centering
  \footnotesize
  \begin{tabular}{c||c|c|c|c||c}
    Task & \inlinecode{dmmp} & \inlinecode{damp} & \inlinecode{dtkp-3} & \inlinecode{dtkp-10} & Baseline \\ \hline
    sum2 & & & & & 21430 (DPL) \\
    sum3 & & & & & 30898 (DPL) \\
    sum4 & & & & & timeout (DPL) \\
    less-than & & & & & 2540 (DPL) \\
    not-3-or-4 & & & & & 3218 (DPL) \\ \hline
    HWF & & & & & \\ \hline
    CLEVR & & & & & -- \\
  \end{tabular}
  \caption{
    Runtime efficiency comparisons.
    Numbers shown are training time (sec) per epoch.
  }
  \label{tab:runtime-efficiency-comparison}
\end{table}


==> figures/scallop-interface.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/scallopy-interface.pdf}
    \caption{Caption for \ours interface}
    \label{fig:scallop-interface}
\end{figure}


==> sections/7-limitations.tex <==
\section{Limitations and Future Work}
\label{sec:limitations}

% \paragraph{Limitations}

% \ours~ is a rule based system that requires programmers to carefully model the relational schema and the rules.
% This is desirable in many cases, when there is a well-defined and constrained problem domain and logical specification.
% However, \ours~ can only be so effective when used in an open-domain setting, such as free-form natural language question answering.
% Take CLEVR VQA as an example: if a user asks ``how many objects are there \textit{between} the two cubes'', the \ours~ program in its current state will be insufficient,
% as there is no definition for the concept ``between''.
% In such case, an end-to-end neural model such as Flamingo \ziyang{cite} will have a better chance answering the question correctly.
% Works in ILP can be employed to create rules and potentially intermediate relations that are needed for reasoning.
% However, more research still needs to be done on relational abstraction over open-domain problems.

% Another limitation of \ours~ is its expressiveness.
% Based on Datalog, \ours~ is not turing complete and hence cannot be used to solve, for example, SAT related problems such as NLSAT \ziyang{cite} and Visual Sudoku \ziyang{cite}.
% We believe \ours~ is capable of solving many real world learning tasks requiring deductive reasoning capability, and to expand the application domain, we want to allow \ours~ to accept complex first-order formulas that require SAT or SMT solving, similar to Formulog \ziyang{cite}.
% This can be done through foreign function interfaces \ziyang{cite evidental tool bus, blah blah}

% \paragraph{Future Work}

% One major direction of future work is to expand the domain of our provenance framework above probabilities.
% In principle, our framework accepts any provenance structure.
% For example, we can tag distributions, observations, and even confidence intervals to each input fact.
% What's even more, latent embeddings can be attached and propagated throughout the reasoning process too.
% Language wise, we want to

% Lastly, we want to expand the application domain of \ours.
% For example in Reinforcement Learning (RL), \ours~ can be utilized to check temporal logic specifications.
% In game playing, \ours~ can be used to enforce logical constraints to help neural networks avoid spurious moves.


==> sections/old-1-introduction.tex <==
\section{Introduction}

Classical algorithms and deep learning embody two prevalent paradigms of modern programming.
Classical algorithms are well suited for exactly defined tasks, such as sorting a list of numbers or finding a shortest path in a graph.
Deep learning on the other hand is well suited for tasks that cannot be performed using classical algorithms, such as detecting objects in an image or parsing text written in natural language.
These tasks are typically specified using a set of input-output training data, and solving them involves learning the parameters (weights) of a deep neural network to fit the data using stochastic gradient descent techniques.

The complementary benefits of these two paradigms have spurred modern applications that demand the capabilities of both.
Examples include question answering \cite{qa}, code completion \cite{codex}, and mathematical problem solving \cite{math}, among many others.
For instance, code completion requires deep learning to comprehend programmer intent from the code context, and classical algorithms to ensure that the generated code is correct.
A natural and fundamental question then is how to program such applications by systematically combining the two paradigms in a single system.

Neuro-symbolic programming is an emerging paradigm that aims to fulfill this goal \cite{swarat}.
A growing body of literature has demonstrated that integrating symbolic knowledge and reasoning with neural architectures yields {\em neuro-symbolic programs} that are more robust, generalizable, data-efficient, and interpretable than either their neural or symbolic counterparts alone.
For instance, consider the task of handwritten formula recognition (HWF) \cite{hwf}, which takes as input a formula as an image, and outputs a number corresponding to the result of evaluating the formula.
An example input-output sample for this task is $\langle x = \hwfsample{figures/hwf_intro}, y = 9 \rangle$.
A neuro-symbolic program for this task might first use a convolutional neural network to extract a sequence of symbols [`5', `+', `8', `/', `2'] from the input image, followed by a classical algorithm to parse the sequence, evaluate the parsed formula using arithmetic operations, and produce the final result $9$.

\todo{Is small-case x and y the right notation for input-output?}
\todo{Make "5 + 8 / 2" look like a HWF.}
\todo{In addition, consider explaining how a strictly neural model would approach this, simultaneously pointing out its flaws and inefficiencies.}
\todo{"In the HWF task, this corresponds to not requiring the user to provide the sequence of symbols in each input image in the training data." This sentence is more or less assumed from the explanation of HWF and can be augmented in that paragraph further with an explanation of the standalone neural approach.}

Despite significant strides in neuro-symbolic techniques, there is a lack of a general-purpose language that is expressive enough for writing a wide range of neuro-symbolic applications, yet efficient enough for training them in an end-to-end manner with only algorithmic supervision, i.e., supervision on observable input-output data.
To this end, this paper presents Scallop, a language for neuro-symbolic programming.
A hallmark of neurosymbolic approaches is the extraction of symbols from raw data using deep neural networks, followed by the ability to manipulate those symbols using {\em differentiable} classical algorithms \cite{todo}.
Thus, a language for neuro-symbolic programming must make three fundamental and inter-dependent design decisions:
\begin{enumerate}
    \item How to explicitly represent symbols extracted from raw data using deep neural networks;
    \item What constructs to support in a high-level language for manipulating the symbols; and
    \item How to automatically and efficiently differentiate programs written using those constructs.
\end{enumerate}
We next describe each of these design decisions in Scallop.

{\bf Relational Data Model.} In Scallop, the primary data structure for representing symbols is a {\em relation}.
Relations are general and can represent arbitrary graphs.
For instance, they can represent {\em scene graphs}, a canonical symbolic representation of images \cite{todo}.
Relations can also represent probability distributions over symbols by tagging tuples with associated probabilities. For instance, in the HWF example, the extracted sequence of symbols may be represented by a binary relation ${\tt token}(i, c)$ where $i$ is the index in the sequence and $c$ is either a digit (`0' through `9') or an arithmetic operator (`+', `-', `*', or `/'):
\[
\footnotesize
\begin{tabular}{llllll}
\multicolumn{5}{l}{{\tt rel token = } \{} \\
   & \sclcode{.95::(0, "5")}, &
     \regcode{.51::(1, "-")}, &
     \sclcode{.82::(2, "8")}, &
     \sclcode{.53::(3, "/")}, &
     \sclcode{.89::(4, "2")}, \\
   & \regcode{.04::(0, "3")}, &
     \sclcode{.43::(1, "+")}, &
     \regcode{.12::(2, "6")}, &
     \regcode{.43::(3, "1")}, &
     \regcode{.09::(4, "7")}, \\
   & ... \\
\}
\end{tabular}
\]
where the tagged-tuple \sclcode{.95::(0, "5")} denotes that the first symbol in the sequence is `5' with probability .95, and so on.\footnote{We use shaded background to highlight correct tuples.  In this example, the symbol at each position in the sequence is the correct one---i.e., has the highest probability of all possible symbols---except for the second one which is a `-' instead of `+'.}
Finally, using a relational representation has important practical benefits stemming from the fact that the relational data model has withstood the test of time \cite{codd}.  In particular, it is the most common representation of structured data, and it enables Scallop's compiler to employ sophisticated optimizations from the literature on relational databases.

\todo{Previous sentence: fine, but a bit awkwardly worded, could be more succinct.  Also, format the tuples better?}
\jiani{Should we mention, as most of the data are stored in the form of relational DB, it opens up the possibility of incorporating the existing knowledge into learning system explicitly.}

{\bf Datalog-based Language.}
A central factor in choosing the language to specify classical algorithms is expressiveness.
While a Turing-complete language like Prolog satisfies this need, it conflicts with our next design choice---the desire to efficiently differentiate programs in that language.
To further illustrate this problem, one epoch of training the HWF program written in DeepProbLog \cite{dpl}, a state-of-the-art neuro-symbolic language based on Prolog, takes \todo{X} minutes on a single sample on average.

Instead, Scallop is based on an extension of Datalog, a declarative logic programming language \cite{datalog}.
While not Turing-complete, it supports a rich set of features that suffice to express common reasoning patterns, such as recursion, aggregation, and negation.
These features enable Scallop to be simultaneously data-efficient and capable of compositional reasoning \cite{hupkes2020compositionality}.
For instance, in the HWF task, recursion is needed to parse the unbounded sequence of symbols in the input formula and to subsequently evaluate it.
Scallop achieves \todo{X}\% accuracy for this task using a training set of only \todo{X} samples, including on instances more complex and diverse than those used for training.

\todo{This is a nice statistic, but it needs to be framed in relation to the performance of other languages.  But more importantly, you need to mention the average runtime on a single sample, like you for DeepProbLog!  Otherwise there is no way for the reading to perceive the efficiency of Scallop! Either you mention the accuracy of DeepProbLog or the running time of Scallop.  But in either case their must be a comparison of the same statistic IMO.}

\todo{Possibly mention disjunction over inputs facts as a feature, which extends Datalog's expressiveness but still limited.  Necessary to choose one out of many outputs of a neural network. Give HWF example (just first column).}
\todo{Should we also illustrate many of these concepts with nice pictures of CLEVR etc.?}

{\bf Differentiable Reasoning.}
The third design decision concerns how to efficiently learn the parameters of the neural components of a Scallop program.
For the HWF task, suppose Scallop computes an output distribution over the numeric result from an input distribution over a sequence of symbols, such as the {\tt token} relation instance above:
\[
{\tt rel\ result\ =\ } \{ \regcode{0.63::(1)}, \sclcode{0.34::(9)}, \regcode{0.02::(2)}, ... \}
\]
In this case, the predicted result $\hat{y} = 1$ (that is, the result with the highest probability of 0.63) is different from the expected result $y = 9$.
This error is caused by the neural network mispredicting the second symbol in the sequence as `-' instead of `+'.
The key challenge lies in computing the gradients of the input probabilities by differentiating the loss function induced by the Datalog program.
For the {\tt token} relation instance above, Scallop computes these gradients as a tensor $[\regcode{0.01}, \regcode{0.32}, \regcode{0.01}, \regcode{0.01}, ..., \regcode{0.01}]$ which localizes the error to the second symbol in the sequence.
These gradients in turn are backpropagated to the parameters of the neural network.

Our key insight to efficiently compute both the output probabilities and the gradients of input probabilities is to leverage {\em provenance semirings} \cite{provenancesemiring}, a theory which extends the discrete semantics of Datalog to define and propagate tags on tuples.
We propose a novel and general framework for specifying semirings in the presence of a rich set of constructs (recursion, aggregation, and negation).  We show how to instantiate the framework with semirings from the literature as well as newer ones, resulting in an extensible library of semirings.
Finally, our evaluation shows that different semirings are suitable for different applications in terms of learning rate and test accuracy, justifying the flexibility of our framework in shaping the loss in diverse applications.
%For the HWF example, the ``top k proof semiring" associates each tuple with a set of upto $k$ proofs, where each proof comprises a set of tuples from the {\tt token} relation whose probabilities are to be learned.

We have implemented a comprehensive toolchain for Scallop in 50 KLOC of Rust that includes a compiler, an interpreter, and Pytorch bindings to integrate Scallop programs with existing machine learning pipelines.
We evaluate Scallop’s expressiveness, usability, and performance using 10 significant neuro-symbolic applications from the literature that span image processing, natural language processing, planning, knowledge graph querying, and their combinations.
Our evaluation demonstrates that Scallop is capable of expressing algorithmic reasoning in diverse and challenging AI tasks, provides an easy-to-use interface for
machine learning programmers to integrate logical domain-specific knowledge, and outperforms state-of-the-art deep neural network models in terms of accuracy and data efficiency.

\todo{Above is a complete repeat of the abstract 2nd para. Consider rewriting this but with all of the aforementioned text to summarize.}

The rest of the paper is organized as follows.
Section \ref{sec:overview} presents an illustrative overview of Scallop.
Section \ref{sec:language} defines the syntax and semantics of Scallop.
Section \ref{sec:framework} presents the reasoning framework.
Section \ref{sec:implementation} describes the implementation of Scallop.
Section \ref{sec:evaluation} empirically evaluates Scallop on a benchmark suite.
Section \ref{sec:limitations} discusses limitations and future work.
Section \ref{sec:related} surveys related work and Section \ref{sec:conclusion} concludes.

